High-Performance Reachability Query Processing under Index Size Restrictions

In this paper, we propose a scalable and highly efficient index structure for the reachability problem over graphs. We build on the well-known node interval labeling scheme where the set of vertices reachable from a particular node is compactly encoded as a collection of node identifier ranges. We impose an explicit bound on the size of the index and flexibly assign approximate reachability ranges to nodes of the graph such that the number of index probes to answer a query is minimized. The resulting tunable index structure generates a better range labeling if the space budget is increased, thus providing a direct control over the trade off between index size and the query processing performance. By using a fast recursive querying method in conjunction with our index structure, we show that in practice, reachability queries can be answered in the order of microseconds on an off-the-shelf computer - even for the case of massive-scale real world graphs. Our claims are supported by an extensive set of experimental results using a multitude of benchmark and real-world web-scale graph datasets.

==> parts/tables/ct-benchmark-vark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32-k1,ferrari-L-s32-k2,ferrari-L-s32-k3,ferrari-L-s32-k5,ferrari-G-s32-k1,ferrari-G-s32-k2,ferrari-G-s32-k3,ferrari-G-s32-k5,grail-k1,grail-k2,grail-k3,grail-k5,pt,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32-k1/.style={column name={\bfseries Ferrari-L (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k2/.style={column name={\bfseries Ferrari-L (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k3/.style={column name={\bfseries Ferrari-L (k=3)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k5/.style={column name={\bfseries Ferrari-L (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k1/.style={column name={\bfseries Ferrari-G (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k2/.style={column name={\bfseries Ferrari-G (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k3/.style={column name={\bfseries Ferrari-G (k=3)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k5/.style={column name={\bfseries Ferrari-G (k=5)}, precision=2, zerofill,
    column type=r},
  columns/grail-k1/.style={column name={\bfseries Grail (k=1)}, precision=2, zerofill, column type=r},
  columns/grail-k2/.style={column name={\bfseries Grail (k=2)}, precision=2, zerofill, column
    type=r},
  columns/grail-k3/.style={column name={\bfseries Grail (k=3)}, precision=2, zerofill, column
    type=r},
  columns/grail-k5/.style={column name={\bfseries Grail (k=5)}, precision=2, zerofill, column type=r},
  columns/pt/.style={column name={\bfseries PathTree}, precision=2, zerofill, column type=r, string replace={nan}{}},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-G-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-L-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 4 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 5 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 6 column grail/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 7 column ferrari-G-s32/.style={postproc cell content/.style={@cellcontent=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-ct-benchmark-vark-table.tex
  ] {data/overall-ct-vark.dat}

==> parts/tables/ct-benchmark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32,ferrari-G-s32,grail,pt,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32/.style={column name={\bfseries Ferrari-L}, precision=2, zerofill, column type=r},
  columns/ferrari-G-s32/.style={column name={\bfseries Ferrari-G}, precision=2, zerofill, column type=r},
  columns/grail/.style={column name={\bfseries Grail}, precision=2, zerofill, column type=r},
  columns/pt/.style={column name={\bfseries PathTree}, precision=2, zerofill, column type=r, string replace={nan}{}},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column grail/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column grail/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column grail/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 4 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 5 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 6 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 7 column ferrari-L-s32/.style={postproc cell content/.style={@cell
 content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-ct-benchmark-table.tex
  ] {data/overall-ct.dat}

==> parts/tables/ct-web-vark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32-k1,ferrari-L-s32-k2,ferrari-L-s32-k5,ferrari-L-s32-k10,ferrari-G-s32-k1,ferrari-G-s32-k2,ferrari-G-s32-k5,ferrari-G-s32-k10,grail-k1,grail-k2,grail-k5,grail-k10,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32-k1/.style={column name={\bfseries Ferrari-L (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k2/.style={column name={\bfseries Ferrari-L (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k5/.style={column name={\bfseries Ferrari-L (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k10/.style={column name={\bfseries Ferrari-L (k=10)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k1/.style={column name={\bfseries Ferrari-G (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k2/.style={column name={\bfseries Ferrari-G (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k5/.style={column name={\bfseries Ferrari-G (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k10/.style={column name={\bfseries Ferrari-G (k=10)}, precision=2, zerofill,
    column type=r},
  columns/grail-k1/.style={column name={\bfseries Grail (k=1)}, precision=2, zerofill, column type=r},
  columns/grail-k2/.style={column name={\bfseries Grail (k=2)}, precision=2, zerofill, column
    type=r},
  columns/grail-k5/.style={column name={\bfseries Grail (k=5)}, precision=2, zerofill, column
    type=r},
  columns/grail-k10/.style={column name={\bfseries Grail (k=10)}, precision=2, zerofill, column type=r},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  outfile=parts/tables/overall-ct-web-vark-table.tex
  ] {data/overall-ct-web-vark.dat}

==> parts/tables/ct-web.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32,ferrari-G-s32,grail,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32/.style={column name={\bfseries Ferrari-L}, precision=2, zerofill, column type=r},
  columns/ferrari-G-s32/.style={column name={\bfseries Ferrari-G}, precision=2, zerofill, column type=r},
  columns/grail/.style={column name={\bfseries Grail}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, fixed, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column grail/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column pwah-8/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column grail/.style={postproc cell content/.style={@cell
 content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-ct-web-table.tex
  ] {data/overall-ct-web.dat}

==> parts/tables/overall-qt-r-table.tex <==
%\begin {tabular}{rrrrrrr}%
\begin {tabular*}{\textwidth}{@{\extracolsep{\fill}}rrrrrrr}%
\toprule \bfseries Dataset&\bfseries Ferrari-L&\bfseries Ferrari-G&\bfseries Grail&\bfseries PathTree&\bfseries Interval&\bfseries PWAH-8\\\midrule %
ArXiV&\pgfutilensuremath {23.69}&\pgfutilensuremath {13.91}&\pgfutilensuremath {100.92}&$\mathbf {\pgfmathprintnumber {3.414}}$&\pgfutilensuremath {4.17}&\pgfutilensuremath {23.22}\\%
Pubmed&\pgfutilensuremath {7.58}&\pgfutilensuremath {4.88}&\pgfutilensuremath {12.27}&$\mathbf {\pgfmathprintnumber {2.758}}$&\pgfutilensuremath {3.16}&\pgfutilensuremath {28.58}\\%
Human&$\mathbf {\pgfmathprintnumber {0.784}}$&$\mathbf {\pgfmathprintnumber {0.777}}$&\pgfutilensuremath {4.98}&\pgfutilensuremath {1.21}&\pgfutilensuremath {1.07}&\pgfutilensuremath {1.06}\\%
GO&\pgfutilensuremath {4.10}&\pgfutilensuremath {2.96}&\pgfutilensuremath {4.83}&$\mathbf {\pgfmathprintnumber {2.038}}$&\pgfutilensuremath {2.47}&\pgfutilensuremath {4.45}\\%
CiteSeer&\pgfutilensuremath {6.13}&\pgfutilensuremath {6.24}&\pgfutilensuremath {8.05}&$\mathbf {\pgfmathprintnumber {5.011}}$&\pgfutilensuremath {8.28}&\pgfutilensuremath {12.39}\\%
CiteSeerX&\pgfutilensuremath {15.88}&\pgfutilensuremath {9.31}&\pgfutilensuremath {41.23}&--&$\mathbf {\pgfmathprintnumber {9.2740}}$&\pgfutilensuremath {21.32}\\%
GO-Uniprot&\pgfutilensuremath {28.30}&\pgfutilensuremath {28.92}&$\mathbf {\pgfmathprintnumber {5.9440}}$&--&\pgfutilensuremath {16.82}&\pgfutilensuremath {48.70}\\%
Cit-Patents&\pgfutilensuremath {778.09}&$\mathbf {\pgfmathprintnumber {502.197}}$&\pgfutilensuremath {578.83}&--&--&\pgfutilensuremath {1{,}514.91}\\\bottomrule %
\end {tabular*}%


==> parts/tables/qt-p-benchmark-vark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32-k1,ferrari-L-s32-k2,ferrari-L-s32-k3,ferrari-L-s32-k5,ferrari-G-s32-k1,ferrari-G-s32-k2,ferrari-G-s32-k3,ferrari-G-s32-k5,grail-k1,grail-k2,grail-k3,grail-k5,pt,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32-k1/.style={column name={\bfseries Ferrari-L (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k2/.style={column name={\bfseries Ferrari-L (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k3/.style={column name={\bfseries Ferrari-L (k=3)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k5/.style={column name={\bfseries Ferrari-L (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k1/.style={column name={\bfseries Ferrari-G (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k2/.style={column name={\bfseries Ferrari-G (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k3/.style={column name={\bfseries Ferrari-G (k=3)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k5/.style={column name={\bfseries Ferrari-G (k=5)}, precision=2, zerofill,
    column type=r},
  columns/grail-k1/.style={column name={\bfseries Grail (k=1)}, precision=2, zerofill, column type=r},
  columns/grail-k2/.style={column name={\bfseries Grail (k=2)}, precision=2, zerofill, column
    type=r},
  columns/grail-k3/.style={column name={\bfseries Grail (k=3)}, precision=2, zerofill, column
    type=r},
  columns/grail-k5/.style={column name={\bfseries Grail (k=5)}, precision=2, zerofill, column type=r},
  columns/pt/.style={column name={\bfseries PathTree}, precision=2, zerofill, column type=r, string replace={nan}{}},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-G-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-L-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 4 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 5 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 6 column grail/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 7 column ferrari-G-s32/.style={postproc cell content/.style={@cellcontent=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-qt-p-benchmark-vark-table.tex
  ] {data/overall-qt-p-vark.dat}

==> parts/tables/qt-p-benchmark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32,ferrari-G-s32,grail,pt,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32/.style={column name={\bfseries Ferrari-L}, precision=2, zerofill, column type=r},
  columns/ferrari-G-s32/.style={column name={\bfseries Ferrari-G}, precision=2, zerofill, column type=r},
  columns/grail/.style={column name={\bfseries Grail}, precision=2, zerofill, column type=r},
  columns/pt/.style={column name={\bfseries PathTree}, precision=2, zerofill, column type=r, string replace={nan}{}},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 4 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 5 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 6 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 7 column pwah-8/.style={postproc cell content/.style={@cell
 content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-qt-p-benchmark-table.tex
  ] {data/overall-qt-p.dat}

==> parts/tables/qt-p-web-vark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32-k1,ferrari-L-s32-k2,ferrari-L-s32-k5,ferrari-L-s32-k10,ferrari-G-s32-k1,ferrari-G-s32-k2,ferrari-G-s32-k5,ferrari-G-s32-k10,grail-k1,grail-k2,grail-k5,grail-k10,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32-k1/.style={column name={\bfseries Ferrari-L (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k2/.style={column name={\bfseries Ferrari-L (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k5/.style={column name={\bfseries Ferrari-L (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k10/.style={column name={\bfseries Ferrari-L (k=10)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k1/.style={column name={\bfseries Ferrari-G (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k2/.style={column name={\bfseries Ferrari-G (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k5/.style={column name={\bfseries Ferrari-G (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k10/.style={column name={\bfseries Ferrari-G (k=1ß)}, precision=2, zerofill,
    column type=r},
  columns/grail-k1/.style={column name={\bfseries Grail (k=1)}, precision=2, zerofill, column type=r},
  columns/grail-k2/.style={column name={\bfseries Grail (k=2)}, precision=2, zerofill, column
    type=r},
  columns/grail-k5/.style={column name={\bfseries Grail (k=5)}, precision=2, zerofill, column
    type=r},
  columns/grail-k10/.style={column name={\bfseries Grail (k=10)}, precision=2, zerofill, column type=r},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  outfile=parts/tables/overall-qt-p-web-vark-table.tex
  ] {data/overall-qt-p-web-vark.dat}

==> parts/tables/qt-p-web.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32,ferrari-G-s32,grail,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32/.style={column name={\bfseries Ferrari-L}, precision=2, zerofill, column type=r},
  columns/ferrari-G-s32/.style={column name={\bfseries Ferrari-G}, precision=2, zerofill, column type=r},
  columns/grail/.style={column name={\bfseries Grail}, precision=2, zerofill, column type=r,string replace={nan}{}},
  %columns/pt/.style={column name={\bfseries PathTree}, precision=2, zerofill, column type=r, string replace={nan}{}},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-G-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column ferrari-G-s32/.style={postproc cell content/.style={@cell
  content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-qt-p-web-table.tex
  ] {data/overall-qt-p-web.dat}

==> parts/tables/qt-r-benchmark-vark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32-k1,ferrari-L-s32-k2,ferrari-L-s32-k3,ferrari-L-s32-k5,ferrari-G-s32-k1,ferrari-G-s32-k2,ferrari-G-s32-k3,ferrari-G-s32-k5,grail-k1,grail-k2,grail-k3,grail-k5,pt,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32-k1/.style={column name={\bfseries Ferrari-L (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k2/.style={column name={\bfseries Ferrari-L (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k3/.style={column name={\bfseries Ferrari-L (k=3)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k5/.style={column name={\bfseries Ferrari-L (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k1/.style={column name={\bfseries Ferrari-G (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k2/.style={column name={\bfseries Ferrari-G (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k3/.style={column name={\bfseries Ferrari-G (k=3)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k5/.style={column name={\bfseries Ferrari-G (k=5)}, precision=2, zerofill,
    column type=r},
  columns/grail-k1/.style={column name={\bfseries Grail (k=1)}, precision=2, zerofill, column type=r},
  columns/grail-k2/.style={column name={\bfseries Grail (k=2)}, precision=2, zerofill, column
    type=r},
  columns/grail-k3/.style={column name={\bfseries Grail (k=3)}, precision=2, zerofill, column
    type=r},
  columns/grail-k5/.style={column name={\bfseries Grail (k=5)}, precision=2, zerofill, column type=r},
  columns/pt/.style={column name={\bfseries PathTree}, precision=2, zerofill, column type=r, string replace={nan}{}},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-G-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-L-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 4 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 5 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 6 column grail/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 7 column ferrari-G-s32/.style={postproc cell content/.style={@cellcontent=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-qt-r-benchmark-vark-table.tex
  ] {data/overall-qt-r-vark.dat}

==> parts/tables/qt-r-benchmark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32,ferrari-G-s32,grail,pt,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32/.style={column name={\bfseries Ferrari-L}, precision=2, zerofill, column type=r},
  columns/ferrari-G-s32/.style={column name={\bfseries Ferrari-G}, precision=2, zerofill, column type=r},
  columns/grail/.style={column name={\bfseries Grail}, precision=2, zerofill, column type=r},
  columns/pt/.style={column name={\bfseries PathTree}, precision=2, zerofill, column type=r, string replace={nan}{}},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-G-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-L-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 4 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 5 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 6 column grail/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 7 column ferrari-G-s32/.style={postproc cell content/.style={@cell
 content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-qt-r-benchmark-table.tex
  ] {data/overall-qt-r.dat}

==> parts/tables/qt-r-web-vark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32-k1,ferrari-L-s32-k2,ferrari-L-s32-k5,ferrari-L-s32-k10,ferrari-G-s32-k1,ferrari-G-s32-k2,ferrari-G-s32-k5,ferrari-G-s32-k10,grail-k1,grail-k2,grail-k5,grail-k10,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32-k1/.style={column name={\bfseries Ferrari-L (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k2/.style={column name={\bfseries Ferrari-L (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k5/.style={column name={\bfseries Ferrari-L (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k10/.style={column name={\bfseries Ferrari-L (k=10)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k1/.style={column name={\bfseries Ferrari-G (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k2/.style={column name={\bfseries Ferrari-G (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k5/.style={column name={\bfseries Ferrari-G (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k10/.style={column name={\bfseries Ferrari-G (k=10)}, precision=2, zerofill,
    column type=r},
  columns/grail-k1/.style={column name={\bfseries Grail (k=1)}, precision=2, zerofill, column type=r},
  columns/grail-k2/.style={column name={\bfseries Grail (k=2)}, precision=2, zerofill, column
    type=r},
  columns/grail-k5/.style={column name={\bfseries Grail (k=5)}, precision=2, zerofill, column
    type=r},
  columns/grail-k10/.style={column name={\bfseries Grail (k=10)}, precision=2, zerofill, column type=r},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  outfile=parts/tables/overall-qt-r-web-vark-table.tex
  ] {data/overall-qt-r-web-vark.dat}

==> parts/tables/qt-r-web.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32,ferrari-G-s32,grail,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32/.style={column name={\bfseries Ferrari-L}, precision=2, zerofill, column type=r},
  columns/ferrari-G-s32/.style={column name={\bfseries Ferrari-G}, precision=2, zerofill, column type=r},
  columns/grail/.style={column name={\bfseries Grail}, precision=2, zerofill, column type=r, string replace={nan}{}},
  %columns/pt/.style={column name={\bfseries PathTree}, precision=2, zerofill, column type=r, string replace={nan}{}},
  columns/pwah-interval/.append style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column pwah-interval/.style={prepoc cell content/.style={precision=2, zerofill}, postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column pwah-interval/.style={prepoc cell content/.style={precision=2, zerofill}, postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-L-s32/.style={prepoc cell content/.style={precision=2, zerofill}, postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column ferrari-L-s32/.style={prepoc cell content/.style={precision=2, zerofill},
  postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-qt-r-web-table.tex
  ] {data/overall-qt-r-web.dat}

==> parts/tables/size-benchmark-vark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32-k1,ferrari-L-s32-k2,ferrari-L-s32-k3,ferrari-L-s32-k5,ferrari-G-s32-k1,ferrari-G-s32-k2,ferrari-G-s32-k3,ferrari-G-s32-k5,grail-k1,grail-k2,grail-k3,grail-k5,pt,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32-k1/.style={column name={\bfseries Ferrari-L (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k2/.style={column name={\bfseries Ferrari-L (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k3/.style={column name={\bfseries Ferrari-L (k=3)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k5/.style={column name={\bfseries Ferrari-L (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k1/.style={column name={\bfseries Ferrari-G (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k2/.style={column name={\bfseries Ferrari-G (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k3/.style={column name={\bfseries Ferrari-G (k=3)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k5/.style={column name={\bfseries Ferrari-G (k=5)}, precision=2, zerofill,
    column type=r},
  columns/grail-k1/.style={column name={\bfseries Grail (k=1)}, precision=2, zerofill, column type=r},
  columns/grail-k2/.style={column name={\bfseries Grail (k=2)}, precision=2, zerofill, column
    type=r},
  columns/grail-k3/.style={column name={\bfseries Grail (k=3)}, precision=2, zerofill, column
    type=r},
  columns/grail-k5/.style={column name={\bfseries Grail (k=5)}, precision=2, zerofill, column type=r},
  columns/pt/.style={column name={\bfseries PathTree}, precision=2, zerofill, column type=r, string replace={nan}{}},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-G-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column ferrari-L-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 4 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 5 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 6 column grail/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 7 column ferrari-G-s32/.style={postproc cell content/.style={@cellcontent=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-size-benchmark-vark-table.tex
  ] {data/overall-size-vark.dat}

==> parts/tables/size-benchmark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32,ferrari-G-s32,grail,pt,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32/.style={column name={\bfseries Ferrari-L}, fixed,  precision=2, zerofill,column type=r},
  columns/ferrari-G-s32/.style={column name={\bfseries Ferrari-G}, fixed,  precision=2, zerofill,column type=r},
  columns/grail/.style={column name={\bfseries Grail}, fixed,  precision=2, zerofill,column type=r},
  columns/pt/.style={column name={\bfseries PathTree}, fixed,  precision=2, zerofill,column type=r, string replace={nan}{}},
  columns/pwah-interval/.style={column name={\bfseries Interval}, fixed,  precision=2, zerofill,column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, fixed,  precision=2, zerofill,column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column ferrari-L-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column ferrari-L-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 4 column pt/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 5 column pwah-8/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 6 column pwah-8/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 7 column ferrari-L-s32/.style={postproc cell content/.style={@cell
 content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-size-benchmark-table.tex
  ] {data/overall-size.dat}

==> parts/tables/size-web-vark.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32-k1,ferrari-L-s32-k2,ferrari-L-s32-k5,ferrari-L-s32-k10,ferrari-G-s32-k1,ferrari-G-s32-k2,ferrari-G-s32-k5,ferrari-G-s32-k10,grail-k1,grail-k2,grail-k5,grail-k10,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32-k1/.style={column name={\bfseries Ferrari-L (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k2/.style={column name={\bfseries Ferrari-L (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k5/.style={column name={\bfseries Ferrari-L (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-L-s32-k10/.style={column name={\bfseries Ferrari-L (k=10)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k1/.style={column name={\bfseries Ferrari-G (k=1)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k2/.style={column name={\bfseries Ferrari-G (k=2)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k5/.style={column name={\bfseries Ferrari-G (k=5)}, precision=2, zerofill,
    column type=r},
  columns/ferrari-G-s32-k10/.style={column name={\bfseries Ferrari-G (k=10)}, precision=2, zerofill,
    column type=r},
  columns/grail-k1/.style={column name={\bfseries Grail (k=1)}, precision=2, zerofill, column type=r},
  columns/grail-k2/.style={column name={\bfseries Grail (k=2)}, precision=2, zerofill, column
    type=r},
  columns/grail-k5/.style={column name={\bfseries Grail (k=5)}, precision=2, zerofill, column
    type=r},
  columns/grail-k10/.style={column name={\bfseries Grail (k=10)}, precision=2, zerofill, column type=r},
  columns/pwah-interval/.style={column name={\bfseries Interval}, precision=2, zerofill, column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, precision=2, zerofill, column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  outfile=parts/tables/overall-size-web-vark-table.tex
  ] {data/overall-size-web-vark.dat}

==> parts/tables/size-web.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
 \pgfplotstabletypeset[
  columns={dataset,ferrari-L-s32,ferrari-G-s32,grail,pwah-interval,pwah-8},
  column type=r,
  columns/dataset/.style={column name={\bfseries Dataset}, string type},
  columns/ferrari-L-s32/.style={column name={\bfseries Ferrari-L}, fixed,  precision=2, zerofill,column type=r},
  columns/ferrari-G-s32/.style={column name={\bfseries Ferrari-G}, fixed,  precision=2, zerofill,column type=r},
  columns/grail/.style={column name={\bfseries Grail}, fixed,  precision=2, zerofill,column type=r,string replace={nan}{}},
  %columns/pt/.style={column name={\bfseries PathTree}, fixed,  precision=2, zerofill,column type=r, string replace={nan}{}},
  columns/pwah-interval/.style={column name={\bfseries Interval}, fixed,  precision=2, zerofill,column type=r,string replace={nan}{}},
  columns/pwah-8/.style={column name={\bfseries PWAH-8}, fixed,  precision=2, zerofill,column type=r,string replace={nan}{}},
  every head row/.style={before row=\toprule, after row=\midrule},
  every last row/.style={after row=\bottomrule},
  empty cells with={--},
  every row 0 column pwah-8/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 1 column ferrari-L-s32/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 2 column pwah-interval/.style={postproc cell content/.style={@cell content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  every row 3 column pwah-8/.style={postproc cell content/.style={@cell
  content=$\mathbf{\pgfmathprintnumber{##1}}$}},
  outfile=parts/tables/overall-size-web-table.tex
  ] {data/overall-size-web.dat}
